Blockchain CAP Theorem Allows User-Dependent Adaptivity and Finality

Longest-chain blockchain protocols, such as Bitcoin, guarantee liveness even when the number of actively participating users is variable, i.e., they are adaptive. However, they are not safe under network partitions, i.e., they do not guarantee finality. On the other hand, classical blockchain protocols, like PBFT, achieve finality but not adaptivity. Indeed, the CAP theorem in the context of blockchains asserts that no protocol can simultaneously offer both adaptivity and finality. We propose a new blockchain protocol, called the checkpointed longest chain, that offers individual users the choice between finality and adaptivity instead of imposing it at a system-wide level. This protocol's salient feature is that it supports two distinct confirmation rules: one that guarantees adaptivity and the other finality. The more optimistic adaptive rule always confirms blocks that are marked as finalized by the more conservative rule, and may possibly confirm more blocks during variable participation levels. Clients (users) make a local choice between the confirmation rules as per their personal preference, while miners follow a fixed block proposal rule that is consistent with both confirmation rules. The proposed protocol has the additional benefit of intrinsic validity: the finalized blocks always lie on a single blockchain, and therefore miners can attest to the validity of transactions while proposing blocks. Our protocol builds on the notion of a finality gadget, a popular technique for adding finality to longest-chain protocols.

==> B_section6.2.tex <==

\section{Checkpointing Properties}
\label{app:property2}


\begin{definition}[Potential starting value for period $p$]
A value $v$ that has been next-voted by $t+1$ honest users for period $p-1$.
\end{definition}

\begin{definition}[Committed value for period $p$]
A value $v$ that has been cert-voted by $2t+1$ users for period $p$.
\end{definition}

\begin{definition}[Potentially committed value for period $p$]
A value $v$ that has been cert-voted by $t+1$ honest users for period $p$.
\end{definition}


\begin{lemma}[Asynchronous Safety]
\label{lem:ba_safe}
Even when the network is partitioned, the protocol ensures safety of the system so that no two honest users will finish one iteration of the protocol with different outputs.
\end{lemma}

\begin{proof}
The following properties hold even during a network partition.
\begin{itemize}
    \item By quorum intersection, as each honest node only soft-votes one value, then at most one value is committed or potentially committed for each period $p$ in one iteration.
    \item If a value $v$ is potentially committed for period $p$, then only $v$ can receive $2t+1$ next-votes for period $p$. Thus, the unique potential starting value for period $p+1$ is $v$.
    \item If a period $p$ has a unique potential starting value $v \neq \perp$, then only $v$ can be committed for period $p$. Moreover, honest nodes will only next-vote $v$ for period $p$, so the unique potential starting value for period $p+1$ is also $v$. Inductively, any future periods $p'>p$ can only have $v$ as a potential starting value. Thus, once a value is potentially committed, it becomes the unique value that can be committed or potentially committed for any future period, and no two honest nodes will finish this iteration of the protocol with different outputs.
    %\textit{\color{red} Add something saying this implies that all users will agree on each committed. block so all committed blocks will be on a chain. }
\end{itemize}


\end{proof}

\begin{lemma}[Asynchronous Deadlock-freedom]
\label{lem:deadlock_free}
As long as messages will be delivered eventually, an honest node can always leave period $p$, either by entering a higher period or meeting the halting condition for the current iteration.
\end{lemma}

\begin{proof}
We first prove that there can never exist $2t+1$ next-votes for two different non-$\perp$ values from the same period $p$ by induction.

Start with $p = 1$. Note that every honest node sets $st^1_i = \perp$ and at most one value (say $v$) could receive more than $2t+1$ soft-votes. Therefore only value $v$ and $\perp$ could potentially receive more than $2t+1$ next-votes in period $1$. Note that it is possible that both $v$ and $\perp$ receive more than $2t+1$ next-votes: all the honest nodes could next-vote for $\perp$ in Step 4 and then next-vote for $v$ in Step 5 after seeing the $2t+1$ soft-votes for $v$.

Assume that the claim holds for period $p-1$ ($p \geq 2$): there exist at most two values each of which has $2t + 1$ next-votes for period $p-1$, and
one of them is necessarily $\perp$. Then there are three possible cases:

\begin{itemize}
    \item Case 1: Only $\perp$ has $2t + 1$ next-votes for period $p-1$. This is the same as the induction basis $p=1$.
    \item Case 2: Only $v$ has $2t+1$ next-votes for period $p-1$. Then in period $p$, every honest node will have starting value $st^p_i = v$, so only $v$ could receive soft-vote and next-vote.
    \item Case 3: Both $\perp$ and $v$ have $2t + 1$ next-votes for period $p-1$. Suppose a new value $v' \neq v$ receives $2t+1$ next-votes for period $p$, then $v'$ must have $2t+1$ soft-votes for period $p$ and at least $t+1$ soft-votes are from honest nodes, which means that at least $t+1$ honest nodes have received $2t + 1$ next-votes for $\perp$ for period $p - 1$ when they enter Step 2. Hence when they enter Step 4, they will next-vote $v'$ or $\perp$ instead of $v$. And they will not next-vote $v$ in Step 5 either. Then $v$ can have at most $t$ next-votes from honest nodes and at most $2t$ next-votes from all nodes for period $p$.
\end{itemize}
 
Therefore, we proved the claim for period $p$. Then we prove the lemma. Note that a node will stuck in period $p$ if and only if no value receives at least $2t+1$ next-votes for period $p$. Then by the previous claim we proved, there are only two possible cases:
\begin{itemize}
    \item Case 1: $\perp$ has $2t + 1$ next-votes for period $p-1$. If no value has at least $2t+1$ soft-votes for period $p$, then every honest node will just next-vote $\perp$ in Step 4 or Step 5 (since $2t+1$ next-votes on $\perp$ for period $p-1$ will eventually reach every honest node). Otherwise if some value $v$ has at least $2t+1$ soft-votes for period $p$, then every honest node will next-vote $v$.
    \item Case 2: Only some value $v$ has $2t+1$ next-votes for period $p-1$. Then in period $p$, every honest node will have starting value $st^p_i = v$, so only $v$ could receive soft-vote and next-vote. And every honest node will next-vote $v$ in Step 4.
\end{itemize}


\end{proof}

\begin{lemma}[Conditional Liveness After GST]
\label{lem:cond_live}
Suppose after time $T$, all honest nodes always have the same values, i.e., their local checkpointed longest chains satisfy common prefix property, then after $\max\{{\rm GST},T\}$, each iteration of Algorand BA will finish within $O(\Delta)$ time. Moreover, all honest nodes finish the same iteration within time $\Delta$ apart. 
%Moreover, only recent inputted values will be outputted.
\end{lemma}

\begin{proof}

Let $N$ be the largest iteration number such that some honest node has committed some value $v$ before GST. Then all honest nodes will receive the certificate for $v$ within time $\Delta$ after GST and they will all enter iteration $N+1$ after some time. If such $N$ does not exist, i.e., no value has been committed by any honest node before GST, then we set $N=0$.

Further, let $p$ be the highest period that some honest user is working on in iteration $N+1$ right before GST is. Then after time $\Delta$, all honest nodes will also start period $p$ as they receive $2t + 1$ next-votes for period $p - 1$. Soon after, some value $v$ (which may be $\perp$) will receive at least $2t+1$ for period p by Lemma \ref{lem:deadlock_free}, and all honest node will all start period $p + 1$ within time $\Delta$ apart.
%Note that if $GST < (N+1)e$, then no honest node enters iteration $N+1$ at GST, but all will start period $1$ of iteration $N+1$ at the beginning of slot $(N+1)e$.

Once all honest nodes start the same period $p$ within time $\Delta$ apart, the network partition seems to have never happened.
Without partition, if all honest nodes have the same value, i.e., after $\max\{{\rm GST},T\}$, the following facts hold:
\begin{itemize}
    \item By Lemma \ref{lem:deadlock_free}, there exist at most two values each of which has $2t+1$ next-votes for every period, and one of them is necessarily $\perp$ if there exist exactly two.
    \item If a period $p$ is reached and the leader is honest, then all honest nodes finish the current iteration in period $p$ by their own time $6\Delta$, with the same output $v \neq \perp$. Moreover, all honest nodes finish within time $\Delta$ apart. Indeed, if there exists a potentially committed value $v$ for period $p-1$, then $v$ will be the unique potential starting value for period $p$. In period $p$, the honest leader proposes $v$ in Step 1 and all honest nodes soft-vote $v$ in Step 2. In Step 3, by their own time $4\Delta$, all honest nodes have cert-voted $v$. Thus all of them finish the current iteration by their own time $6\Delta$, with output $v$. Otherwise if there is no potentially committed value in period $p-1$, then the leader of period $p$ may propose its private input $v'$ or a value $v \neq \perp$ for which it has seen $2t+1$ next-votes from period $p-1$. In the first case, all honest nodes will soft-vote $v'$ in Step 2 as they all see $2t+1$ next-votes for $\perp$ from period $p-1$; in the second case, all honest nodes will soft-vote v in Step 2 either by condition 1 or condition 2. In both cases, all honest nodes will cert-vote the same value in Step 3 by their own time $4\Delta$ and finish the current iteration with that value by their own time $6\Delta$.
    \item If a period $p$ is reached and there is no committed value for period $p$ (which only happens if the leader is malicious), then all honest nodes move to period $p+1$ by their own time $8\Delta$, and they move within time $\Delta$ apart. Note that the honest nodes may start period $p$ not at the same time but within time $\Delta$ apart. Indeed, if no honest node has cert-voted in Step 3, then all honest nodes next-vote a common starting value $v$ in Step 4 if no one has seen $2t+1$ next-votes for $\perp$ for period $p-1$, or else all honest nodes next-vote $\perp$ in Step 4 or Step 5. In both cases, they all see these next-votes and move to period $p+1$ by their own time $8\Delta$. If at least one honest node has cert-voted a value $v$ in Step 3, then $v$ must have received $2t + 1$ soft-votes and no other value could have these many soft-votes by quorum intersection. Thus only $v$ could have received cert-votes. Since those honest nodes have helped rebroadcasting the soft-votes for $v$ by their own time $4\Delta$, all honest nodes see $2t+ 1$ soft-votes for $v$ by their own time $6\Delta$. Thus all honest nodes next-vote $v$ either in Step 4 or Step 5 by their own time $6\Delta$, and all see $2t+1$ next-votes for the same value by their own time $8\Delta$. Note that some honest nodes may have next-voted for $\perp$ in Step 4 as well, thus there may also exist $2t + 1$ next-votes for $\perp$.
    \item Combining the above facts together, since the leader in each period is honest with probability $> 2/3$, one iteration takes in expectation at most 1.5 periods and at most $10\Delta$ time. Moreover, all honest nodes finish within time $\Delta$ apart.
\end{itemize}

\end{proof} 

The liveness property showed in Lemma \ref{lem:cond_live} conditions on the assumption that all honest nodes will have the same values after some time $T$. However, this assumption may not hold right after GST as the adversary could have a bank of private blocks that can be used to break the common prefix property. During this stage, Algorand BA may still commit some values in favor of the adversary (eg., the adversary sends its favorite chain to all honest nodes). But if the committed value is too old in the sense that no honest node has that checkpointed block in its local longest chain for a long time, then all honest blocks mined during this time interval could be potentially wasted as they are not extending the last checkpoint. Fortunately, we show that Algorand BA with our cautious modification won't let this happen in the following lemma. 


%\xw{The conjecture that the state can remain in $\{v, \perp\}$ for the same $v$ from period $p$ to period $p+1$, only when the leader of period $p$ is malicious, is wrong. Moreover, I found a perpetual liveness attack. Hence, I propose the following modification on the protocol and also a slightly weaker statement (but should be good enough for us).}

%Modification: in Step 2 condition 1, $i$ soft-votes the value $v$ proposed by the leader of that period if (it hears of it) AND (the value is VALID OR $i$ has received $2t+1$ next-votes for $v$ for period $p-1$), OR else it soft-votes $\perp$.

\begin{lemma}
\label{lem:recent}
After GST, if one honest node commits a value $v$ in one iteration at time $t$, then $v$ must have been the input value held by at least one honest node at time no earlier than $t - 8D\Delta$, where $D \sim \rm{Geo}(p)$ with $p>2/3$ is the fraction of honest nodes.
\end{lemma}


\begin{proof}
For a fixed iteration, We define $V_p$ to be the set of potential starting values for period $p$. Then $V_1 = \{ \perp \}$ and also by Lemma \ref{lem:deadlock_free}, we have $1 \leq |V_p| \leq 2$, and $\perp \in V_p$ if $|V_p| = 2$ for all $p$. Note that $V_p = \{v, \perp\}$ is an bad set as $v$ may be an outdated value. Then we show that the state won't remain in $\{v, \perp\}$ for the same $v$ for a long time. %Otherwise the state will turn to $\{\perp\}$, $\{v\}$, $\{v'\}$, or $\{v', \perp\}$ where $v'$ is a new value.

Suppose the leader of period $p$ is honest and no honest node has value $v$ for period $p$, then we have the following two cases.
\begin{itemize}
    \item Case 1: if the leader of period $p$ has received $2t+1$ next-votes for $\perp$ for period $p-1$ at the beginning of Step 1, then it will propose $v' \neq v$. Further no honest node will soft-vote or next-vote $v$. Therefore, the state of period $p+1$ will be $\{\perp\}$, $\{v'\}$, or $\{v', \perp\}$.
    \item Case 2: if the leader of period $p$ has received $2t+1$ next-votes only for $v$ for period $p-1$ at the beginning of Step 1, then it will propose $v$. Further every honest node will soft-vote $v$ in Step 2 either by condition 1 or condition 2. Therefore, $v$ will be committed in period $p$.
\end{itemize}

Therefore, after GST, the state won't remain in $\{v, \perp\}$ for the same $v$ from period $p$ to period $p+1$, if the leader of period $p$ is honest and no honest node has value $v$ for period $p$. By Lemma \ref{lem:cond_live}, we know that after GST each period (even with a malicious leader) will finish in $8\Delta$ time. Combining these facts together, we can conclude the lemma.

\end{proof}

